NAIPv2: Debiased Pairwise Learning for Efficient Paper Quality Estimation

The ability to estimate the quality of scientific papers is central to how both humans and AI systems will advance scientific knowledge in the future. However, existing LLM-based estimation methods suffer from high inference cost, whereas the faster direct score regression approach is limited by scale inconsistencies. We present NAIPv2, a debiased and efficient framework for paper quality estimation. NAIPv2 employs pairwise learning within domain-year groups to reduce inconsistencies in reviewer ratings and introduces the Review Tendency Signal (RTS) as a probabilistic integration of reviewer scores and confidences. To support training and evaluation, we further construct NAIDv2, a large-scale dataset of 24,276 ICLR submissions enriched with metadata and detailed structured content. Trained on pairwise comparisons but enabling efficient pointwise prediction at deployment, NAIPv2 achieves state-of-the-art performance (78.2% AUC, 0.432 Spearman), while maintaining scalable, linear-time efficiency at inference. Notably, on unseen NeurIPS submissions, it further demonstrates strong generalization, with predicted scores increasing consistently across decision categories from Rejected to Oral. These findings establish NAIPv2 as a debiased and scalable framework for automated paper quality estimation, marking a step toward future scientific intelligence systems. Code and dataset are released at sway.cloud.microsoft/Pr42npP80MfPhvj8.

==> tables/comparison_cur_learning.tex <==
% \begin{figure}[t]
% \begin{minipage}{0.48\linewidth}
%   \centering
%   % 占位图
%   \fbox{\rule[-.8cm]{0cm}{5cm} \rule[-.8cm]{6cm}{0cm}}
%   \caption{Sample figure caption.}
%   \label{fig:sample}
% \end{minipage}\hfill
% \begin{minipage}{0.48\linewidth}
%   \centering
%   \begin{tabular}{lccc}
%   \hline
%   \textbf{Strategy} & \textbf{AUC} & \textbf{NDCG} & \textbf{Spearman} \\
%   \hline
%   xx & 0.XXX & 0.XXX & 0.XXX \\
%   xx                 & 0.XXX & 0.XXX & 0.XXX \\
%   xx & 0.XXX & 0.XXX & 0.XXX \\
%   \hline
%   \end{tabular}
%   \captionof{table}{Comparison of different curriculum learning strategies.}
%   \label{tab:curriculum}
% \end{minipage}
% \end{figure}

